WANDR: Intention-guided Human Motion Generation

Synthesizing natural human motions that enable a 3D human avatar to walk and reach for arbitrary goals in 3D space remains an unsolved problem with many applications. Existing methods (data-driven or using reinforcement learning) are limited in terms of generalization and motion naturalness. A primary obstacle is the scarcity of training data that combines locomotion with goal reaching. To address this, we introduce WANDR, a data-driven model that takes an avatar's initial pose and a goal's 3D position and generates natural human motions that place the end effector (wrist) on the goal location. To solve this, we introduce novel intention features that drive rich goal-oriented movement. Intention guides the agent to the goal, and interactively adapts the generation to novel situations without needing to define sub-goals or the entire motion path. Crucially, intention allows training on datasets that have goal-oriented motions as well as those that do not. WANDR is a conditional Variational Auto-Encoder (c-VAE), which we train using the AMASS and CIRCLE datasets. We evaluate our method extensively and demonstrate its ability to generate natural and long-term motions that reach 3D goals and generalize to unseen goal locations. Our models and code are available for research purposes at wandr.is.tue.mpg.de.

==> supmat/figures/inbetween.tex <==
\begin{figure*}[!h]
    \centering
    \includegraphics[width= 1.\textwidth, trim=0cm 0cm 0cm 0cm]{figures/traj_following.png}
    \caption{Demonstration of motion in-betweening during goal reaching, highlighting \methodname's capability to generate motions that conform to intermediate body poses while progressing towards a goal.}
    \label{fig:motion_inbetweening}
    % \vspace{-3mm}
\end{figure*}

==> supmat/figures/moving_goal.tex <==
\begin{figure*}[!h]
    \centering
    \includegraphics[width= .9\textwidth, trim=0cm 0cm 0cm 0cm]{figures/moving_goal_dummy.png}
    \caption{moving goal reaching}
    \label{fig:moving_goal}
    % \vspace{-3mm}
\end{figure*}



==> supmat/tabs/optimization_table.tex <==
\begin{table}[tb]
\centering
% \small
% \resizebox{1.\linewidth}{!}{
\begin{tabular}{l|ccc}
\Xhline{2\arrayrulewidth}
\textbf{} & \textbf{SR $\uparrow$} & \textbf{FS $\downarrow$} & \textbf{DTG (cm) $\downarrow$} \\
\hline
\methodname        & KK\% & KK\% & KK \\
\methodname+opt.        & KK\% & KK\% & KK \\
\methodname+post opt.        & KK\% & KK\% & KK \\
\Xhline{2\arrayrulewidth}
\end{tabular}
% }
\caption{}
\vspace{-3mm}
\label{tab:optimization}
\end{table}
